Efficient Distributed Community Detection in the Stochastic Block Model

Designing effective algorithms for community detection is an important and challenging problem in {\em large-scale} graphs, studied extensively in the literature. Various solutions have been proposed, but many of them are centralized with expensive procedures (requiring full knowledge of the input graph) and have a large running time. In this paper, we present a distributed algorithm for community detection in the {\em stochastic block model} (also called {\em planted partition model}), a widely-studied and canonical random graph model for community detection and clustering. Our algorithm called {\em CDRW(Community Detection by Random Walks)} is based on random walks, and is localized and lightweight, and easy to implement. A novel feature of the algorithm is that it uses the concept of {\em local mixing time} to identify the community around a given node. We present a rigorous theoretical analysis that shows that the algorithm can accurately identify the communities in the stochastic block model and characterize the model parameters where the algorithm works. We also present experimental results that validate our theoretical analysis. We also analyze the performance of our distributed algorithm under the CONGEST distributed model as well as the $k$-machine model, a model for large-scale distributed computations, and show that it can be efficiently implemented.

==> parts/cdralgorithm.tex <==
\subsection{Community Detection  by Sparsification-Triangulation (CDST)}
\label{sec:cdr-algo}
We propose another localized algorithm (cf. Algorithm~\ref{alg:cdr}) in which we exploit the small-world property of the graphs to detect communities. This algorithm works well in the real world networks, especially in graphs with large clustering coefficients. The main idea behind the algorithm is to remove inter community edges (called {\em sparsification}) and add them as intra community ones (called {\em triangulation}), which essentially improves the community structure of a graph. These two ideas, namely, {\em sparsification} and {\em triangulation}  are adapted from the papers \cite{satuluri2011local, satuluri2012scalable} and \cite{haeupler2012discovery} respectively. We call the described removal and adding of edges as a {\em reorientation} process. 
\par
The algorithm takes an undirected graph $G$ and a tuning parameter $\alpha$ as input and returns a set of communities. The parameter $\alpha$ controls the number of edges being removed from a node. The value of $\alpha$ will be fixed using the experimental analysis. The algorithm runs in synchronous communication rounds. In each round, every node calculates {\em strength} of its adjacent edges. Then nodes remove their low strength edges (if any) and add those edges as intra community edge via the triangulation method. This {\em reorientation} process finishes in $O(n)$ time, described later, resulting in separation of communities. The algorithm as we call it in short {\em CDST} algorithm, finally returns connected components of the graph as its detected communities.
\par 
The strength or weight of an edge $e(u, v)$ is denoted by $w[e(u,v)]$ and is calculated using Jaccard similarity between neighbors of $u$ and $v$. It is the ratio between the number of common neighbors of $u$ and $v$ and the union of their neighbors, i.e., $w[e(u,v)] = \frac{|\Gamma(u) \cap \Gamma(v)|}{|\Gamma(u) \cup \Gamma(v)|}$ where $\Gamma(v)=\{u\in V|(v, u)\in E\}$ is the neighbors of $v$. Since edge density inside a community is higher compared to inter community edges, it is likely that  the nodes inside a community have more common neighbors. This gives higher strength value for the edges inside a community than the inter community edges. As a consequence, mostly the inter community edges are selected to be reoriented. A node $v$ needs to have $\Gamma(u)$ in order to calculate exact strength of its edge $e(v, u)$ which would be expensive to exchange those information. We use a hashing technique called minwise independent permutations  or ({\em minhash}) \cite{broder2000min} to approximate the strength of each edge (see \cite[Section 3.1]{satuluri2011local} for the details). 
\par
At each round $r$, CDST calculates the ratio $\frac{\alpha}{r}$. This ratio decreases as the round $r$ increases and cools down the fraction of (adjacent) edges being removed from a node. For this, a variable $count$, which is the minimum between $d(v)-1$ and $\frac{\alpha}{r}\cdot d(v)$, is defined to control the number of edges to be removed from a node. By doing so, the algorithm makes sure to not remove all the adjacent edges of a node and avoid isolating nodes from their community. The higher the $\alpha$ value, the higher the fraction of edges being reoriented at each round. In fact, $\alpha$ measures the fraction of inter community edges and $1-\alpha$ measures the fraction of intra community edges of a node. A higher value of $\alpha$ helps the algorithm to remove more inter community edges and hence make the algorithm faster in identifying the communities. On the other side, a higher $\alpha$ value may choose intra community edges to be reoriented which is not a favored event. This means we have to tune $\alpha$ to as high value as we can while not decreasing the accuracy of the algorithm. The running rounds of CDST will finish in $O(d(v))$ time for each node $v$ because the control variable $count$ becomes zero at $O(d(v))$ time as $r$ increases. The general order for finishing of rounds on all nodes is then $O(\Delta)$, the degree of graph $G$ which can be $O(n)$.

%The proposed algorithm can be extended to find hierarchal communities as well. By repetitively applying CDST algorithm over an induced subgraph of an identified community, we can detect more in depth hierarchical communities. \anis{not clear! what is "hierarchal communities"? Is it standard? else, we have to define it here} %By induced subgraph we mean a subgraph composed by the nodes of a community and all the edges between those nodes from the original graph. \anis{I remove the definition of induced subgraph. This we used before!!} 
%We leave exploring it as a future exploration. \anis{overall: this small paragraph is not clear to me!}
\onlyLong{
 \par
 \noindent \textbf{Run Time Analysis of the CDST algorithm:}\anis{this is not correct until we have the complete algorithm. For the submission version we may remove this run time analysis!}
 It takes $\Theta(\Delta)$ rounds for the algorithm to finish where $\Delta$ is the degree of the graph. In general it becomes $O(n)$ because the degree of a graph can be $n$. The space complexity is in total $\Theta(|E|)$ because the CDST algorithm does not increase the number of edges. Also each node requires only $\Theta(\Delta)$ space which is very efficient for space complexity of each node of the graph.
 \MyRemark{need to discuss and verify its correctness}
 Message complexity could in total be high, $O(n^2\cdot m)$, if we calculate the strength of edges naively. Utilizing minhash technique, we obtain a good estimation of edges' strength in constant time $c$, with big enough value of $c$ \cite[Proposition 4]{satuluri2011local}. This results in $O(n \cdot m)$ message complexity in total.
}
 
\begin{algorithm}[h]
	%\algsetup{linenosize=\tiny}
	\small %\small, \footnotesize, \scriptsize, or \tiny
	\caption{Community Detection  by Sparsification-Triangulation (CDST), pseudocode for each node $v\in V$.}
	\label{alg:cdr}
	\textbf{Input:} An undirected graph $G = (V, E)$, parameter $\alpha$.\\
	\textbf{Output:} Set of Communities
	\begin{algorithmic}[1]
		\For{round $r = 1, 2 \dots d(v)$}
			\State $count \gets \min\{d(v)-1,\, (\frac{\alpha}{r}) \cdot d(v)\}$
			\If{$count>0$}
				\For{$u\in \Gamma(v)$}
					\State $w[e(v, u)] \gets \frac{|\Gamma(u) \cap \Gamma(v)|}{|\Gamma(u) \cup \Gamma(v)|}$
				\EndFor
			\State Sort $w$ by edges' strength.
			\State \Call{SprsTriag}{$G, w[1 \dots count]$}
		\Else
			\State Break for loop
		\EndIf
		\EndFor
		\State \textbf{Return} Connected component of $G$ as communities.
		\item[]
		\Procedure{$SprsTriag$}{Graph $G(V,E)$, $w$}
			\State $D \gets \emptyset$
			\For{$e(v, u) \in w$} \Comment{Sparsification process}
				\If{$d(u)>1$}
					\State Remove edge $e(v, u)$ from $E$.
					\State $D \gets D \cup e(v,u)$
				\EndIf
			\EndFor
			\For{$i=1 \dots |D|$} \Comment{Triangulation process}
			\label{reknitting-for}
				\If{$d(v) \geq 2$}
					\State Randomly sample two nodes of $x,y \in \Gamma(v)$
					\If{$e(x, y) \notin E$}
						\State Add $e(x, y)$ to $E$.
						\State Jump to line \ref{reknitting-for} and continue the for loop 
					\EndIf
				\EndIf
				\State Randomly sample $u \in \Gamma(v)$ and then $y \in \Gamma(u)$.
				\State Add $e(v, y)$ to $E$.
			\EndFor
		\EndProcedure
	\end{algorithmic}
\end{algorithm}

==> parts/experimentalresults.tex <==
\section{Experimental Results}
In this section, we show the empirical results of running Algorithm \ref{alg:cdrw} on two types of synthetic graphs, Random Graphs $G_{np}$ and Stochastic Planted Random Graphs $G_{npq}$.
We set $p=\frac{c\log n}{n}$ where $c=2$ for generating $G_{np}$ graphs. Then, we pick a random node from the graph and run our algorithm \ref{alg:cdrw} on it. All the node of a random graph belongs to one community as the ground truth. We use Jaccard similarity to measure the accuracy of our algorithm.  In Figure \ref{fig:mixgnp} we show accuracy of our algorithm on different sizes of random graphs. Our results show that its accuracy is getting close to $1$ as the size of the graph increases.
\par
For the Stochastic Planted Random Graphs $G_{npq}$ , we set $p=\frac{c\log n}{n}$, where $c=2$, same as for the random graph. We set $n=1024$ and $q=0.1/n$ and change the number of parts, $k$, between $2$ and $32$. Then the size of a $G_{npq}$ graph is $kn$, $2048$ for two part one. Our results show that our method extracts more than $82\%$ of a node's community members. When the number of parts increases, our algorithm's accuracy decreases which is a natural thing to happen because of a decrease in the conductance parameter of each community.
\par
As mentioned in \cite{fortunato2016community}, there is mismatch between topological and annotated communities. Also community sizes are different in real world graphs.\\
There are many different metrics to measure quality of detected communities, look at \cite{chakraborty2017metrics} for a survey. We use modularity defined in \cite{clauset2004finding}. Colin et al. gave an analytical study on this metric \cite{mcdiarmid2018modularity}.
\par
It has been proven that modularity optimization methods have a resolution limit \cite{fortunato2007resolution} where small sized communities missed and merged into bigger communities. Some approaches such as using hierarchical clustering in \cite{blondel2008fast} or providing a tuning parameter to the algorithm in \cite{traag2011narrow} is proposed. Infomap \cite{bohlin2014community} mitigates this resolution limitation by using a multilevel map equation.

\begin{figure}[t!]
	\centering
	\begin{subfigure}[b]{0.5\columnwidth}
		\centering
		\includegraphics[height=2.7in]{./parts/figs/mixingsize-Gnp1024.pdf}
		\caption{Mixing set size of a random graph of size $n=1024$ and $c=2$.}
	\end{subfigure}%
	~ 
	\begin{subfigure}[b]{0.5\columnwidth}
		\centering
		\includegraphics[height=2.7in]{./parts/figs/mixingsize-Gnpq,n=256,k=4.pdf}
		\caption{Mixing set size of a planted random graph of $4$ parts, each of size $n=1024$ and $q=0.6/n$.}
	\end{subfigure}
	\caption{The size of mixing set after each walk. It shows the range size of mixing set after a walk which can overlap or there could be a gap between them.}
\end{figure}

\begin{figure}[h]
	\centering
	\includegraphics[]{./parts/figs/mixing-gnp.pdf}
	\caption{Axis $x$ shows $n$, the size of the random graphs and axis $y$ shows accuracy. The accuracy of Jaccard similarity of founded community by local mixing method in algorithm \ref{alg:cdrw} and ground truth community gets close to $1$ when the size of graph increases.}
	\label{fig:mixgnp}
\end{figure}

\begin{figure}[h]
	\centering
	%\includegraphics[]{./figs/mixing-gnpq1024k.png}
	\includegraphics[]{./figs/mixing-gnpq.pdf}
	\caption{Axis $x$ shows $k$, the number of parts of $G_{npq}$ graphs. The size of each part is equal to $n$. It shows that our algorithm correctly finds more then $80\%$ members of a community a node belongs to.}
	\label{fig:mixgnpq}
\end{figure}


==> parts/localmixingalgorithmruntime.tex <==
\noindent{\textbf{Run Time:}}\\
%% Running Time Discussion %%%%
It is shown in \cite{MP18} that local mixing time can be computed in $O(\tau^{loc})\log^3 n$ time in a regular graph, where $\tau^{loc}$ is the local mixing time of the graph corresponding to a source node $s$. The local mixing time algorithm in \cite{MP18} uses several binary search (such as on the length of the random walk, on the size of the mixing set, to find $|S|$ smallest $x_u$ values) to achieve the time complexity. Their algorithm essentially computes local mixing set by checking if there is a mixing set of certain size in each step of the random walk. Using the similar ideas and analysis, our algorithm computes the community $V_1$ in $O(\log^4 n)$ time in $G_{np}$, since $\tau^{loc}$ becomes the mixing time of $G_{np}$ which is $O(\log n)$. 
\par
When a graph has multiple $k$ communities such as in PPM graphs, CDRW algorithm detects communities one by one. So the run time would be $k$ times of detecting each community which is a $G{\frac{n}{k}p}$ random graph. It results in time $O(k \log^4 n)$.

